Domain Adaptive and Generalizable Network Architectures and Training Strategies for Semantic Image Segmentation

Unsupervised domain adaptation (UDA) and domain generalization (DG) enable machine learning models trained on a source domain to perform well on unlabeled or even unseen target domains. As previous UDA&DG semantic segmentation methods are mostly based on outdated networks, we benchmark more recent architectures, reveal the potential of Transformers, and design the DAFormer network tailored for UDA&DG. It is enabled by three training strategies to avoid overfitting to the source domain: While (1) Rare Class Sampling mitigates the bias toward common source domain classes, (2) a Thing-Class ImageNet Feature Distance and (3) a learning rate warmup promote feature transfer from ImageNet pretraining. As UDA&DG are usually GPU memory intensive, most previous methods downscale or crop images. However, low-resolution predictions often fail to preserve fine details while models trained with cropped images fall short in capturing long-range, domain-robust context information. Therefore, we propose HRDA, a multi-resolution framework for UDA&DG, that combines the strengths of small high-resolution crops to preserve fine segmentation details and large low-resolution crops to capture long-range context dependencies with a learned scale attention. DAFormer and HRDA significantly improve the state-of-the-art UDA&DG by more than 10 mIoU on 5 different benchmarks. The implementation is available at https://github.com/lhoyer/HRDA.

==> tables/hrda_other_uda.tex <==
\begin{table}[tb]
\centering
\caption{HRDA applied to different UDA methods on GTA$\rightarrow$Cityscapes.}
\label{tab:other_uda}
\setlength{\tabcolsep}{3pt}
\footnotesize
\begin{tabular}{lllll}
\toprule
                          UDA Method &                           Network &       w/o HRDA &        w/ HRDA & Diff. \\
\midrule
Entropy Min. \cite{vu2019advent} &  DeepLabV2 \cite{chen2017deeplab} & 44.3\spm{0.4} & 46.7\spm{1.2} &        +2.4 \\
Adversarial \cite{tsai2018learning} &  DeepLabV2 \cite{chen2017deeplab} & 44.2\spm{0.1} & 47.1\spm{1.0} &        +2.9 \\
DACS \cite{tranheden2021dacs} &  DeepLabV2 \cite{chen2017deeplab} & 53.9\spm{0.6} & 59.4\spm{1.2} &        +5.5 \\
DAFormer & DeepLabV2 \cite{chen2017deeplab} & 56.0\spm{0.5}  & 63.0\spm{0.4} & +7.0     \\
DAFormer & DAFormer & 68.3\spm{0.5} & 73.8\spm{0.3} &        +5.5 \\
\bottomrule
\end{tabular}
\end{table}
